Materials loss measurements using superconducting microwave resonators

The performance of superconducting circuits for quantum computing is limited by materials losses. In particular, coherence times are typically bounded by two-level system (TLS) losses at single photon powers and millikelvin temperatures. The identification of low loss fabrication techniques, materials, and thin film dielectrics is critical to achieving scalable architectures for superconducting quantum computing. Superconducting microwave resonators provide a convenient qubit proxy for assessing performance and studying TLS loss and other mechanisms relevant to superconducting circuits such as non-equilibrium quasiparticles and magnetic flux vortices. In this review article, we provide an overview of considerations for designing accurate resonator experiments to characterize loss, including applicable types of loss, cryogenic setup, device design, and methods for extracting material and interface losses, summarizing techniques that have been evolving for over two decades. Results from measurements of a wide variety of materials and processes are also summarized. Lastly, we present recommendations for the reporting of loss data from superconducting microwave resonators to facilitate materials comparisons across the field.

==> Loss_0422.tex <==
\section{\label{sec:losses}Losses in Superconducting Microwave Resonators}

Superconducting resonators, while low loss, nevertheless suffer from various forms of intrinsic loss. Characterizing the origins of that loss is the subject of much ongoing research. The dependence of resonator loss on experimental conditions such as applied power and temperature can be used to allocate the loss to a handful of mechanisms.

For an ideal superconducting resonator, the only intrinsic loss is the loss due to thermally excited quasiparticles, which is reduced exponentially as the bath temperature approaches zero. According to Mattis-Bardeen theory \citep{Mattis1958}, the internal quality factor reaches $Q_i>10^7$ for $T < T_c/20$ which is a condition easily satisfied at the base temperature of a dilution refrigerator (DR) or an adiabatic demagnetization refrigerator (ADR). 

In practice, $Q_i$ is dominated by other losses and exhibit loss tangents in the  $10^{-5}$ to $10^{-6}$ range. In addition to being sources of dissipation and degradation of resonator performance, these loss mechanisms are also sources of decoherence in qubit applications as well as sources of noise in superconducting detector applications. For these reasons, considerable effort has been made in understanding the resonator loss mechanisms and reducing their negative effects over the past two decades. 

Resonator loss mechanisms that are most important to quantum circuits include two-level systems (TLS), radiation, vortices, and quasiparticles originating from stray infrared (IR) light and microwave-induced pair-breaking.

\begin{table}
\centering`
\begin{ruledtabular}
\begin{tabular}{cccccc}
    Loss & L or C & Power & Temperature & Frequency & Geometry  \\
    \hline
    TLS & C & - & - & + & -\\
    qp-IR & L & No & No &   &  \\
    qp-$\mu$w & L & +& + & + &   \\
    radiation & L & No & No & + & + \\
    vortex & L & No & + & + & +\\
\end{tabular}
\end{ruledtabular}
\caption{Summary of resonator loss mechanisms and their properties. Column 2 lists whether the loss is associated with the capacitor or inductor part of the resonators. In column 3 to 6, a plus (minus) sign indicated that the loss increase (decrease) with power/temperature/frequency/geometrical dimension. A blank indicates a property that is unknown or not studied.}
\label{tab:losssummary}
\end{table}

Table~\ref{tab:losssummary} gives a summary of common loss types with their important properties. As can be seen from this table that only TLS loss is associated with the capacitor of the resonator while the other loss mechanisms are associated with the inductor. This is because TLS have electrical dipole moments and couple to the electric field, while the other losses are coupled or related to the current in the resonator. 

\begin{figure}[t]
    \centering
    \includegraphics[width = \linewidth]{loss.pdf}
    \caption{Loss mechanisms in superconducting microwave resonators.}
    \label{fig:losssummary}
\end{figure}

Fig.~\ref{fig:losssummary} shows the power dependence as well as relative contributions from each loss channel in a superconducting resonator. The loss due to IR light, radiation and vortex are power independent and can usually be suppressed to an unimportant level ($Q_i\gtrsim 10^6$) by the use of mitigation strategies. Because of its power dependence, TLS loss dominates the total loss at single photon power, where quantum computers operate, while the microwave-inducted quasiparticle loss dominates at high power, where kinetic inductance detectors operate. This review is oriented towards quantum computing applications and therefore we focus on the TLS loss in this review.

\subsection{TLS Loss}
%physical origin\\
Amorphous solids exhibit very different thermal, acoustic, and dielectric properties from crystalline solids at low temperatures, which can be modeled by the two-level system (TLS) model introduced by \cite{Phillips} and \cite{Anderson1972} in the 1970s. Although the microscopic nature of TLS is still unclear \citep{Muller2017}, it is thought that a group of one or more atoms in a disordered solid can tunnel between two sites, giving rise to a broad spectrum of tunneling states in amorphous solids. As first showed by \cite{Martinis2005}, TLS in deposited dielectrics such as SiO2 and SiN is a significant source of loss and decoherence in superconducting quantum circuits. Gao showed that even for a superconducting resonator on crystalline Si without deposited amorphous dielectric, TLS on surfaces and interfaces still dominate resonator internal loss \citep{Gao2008b} and is responsible for excess frequency noise observed in these resonators \citep{Gao2007}. Since then, TLS induced loss, decoherence and noise has been an active area of research. 

\begin{figure}[t]
    \centering
    \includegraphics[width = \linewidth]{TLSTheoCurve.pdf}
    \caption{Theoretical curves of a) TLS loss v.s. power and b) temperature dependence of loss (solid) and frequency shift (dashed).}
    \label{fig:TLSTheoCurves}
\end{figure}

According to the TLS model, TLS induce loss $\tan{\delta_{TLS}}$ and frequency shift $\Delta f/f_0$ to a resonator given by \citep{GaoThesis}
\begin{eqnarray}
\tan{\delta_{TLS}} &=& F \tan{\delta_{TLS}^0} \frac{\tanh(\frac{\hbar \omega_0}{ 2 k_B T})}{\sqrt{1 + |E/E_c|^2}},\label{eqn:TLSloss}\\
\frac{\Delta f}{f_0} &=& -\frac{F \tan{\delta_{TLS}^0}}{\pi}[\Re{\Phi(\frac{1}{2}+\frac{1}{2 \pi i}\frac{\hbar \omega}{k T}) - \log{\frac{\hbar \omega}{k T}}}], \label{eqn:TLSfreqshift}
\end{eqnarray}
where $\tan{\delta_{TLS}}$ is the intrinsic TLS loss tangent, $E_c$ is the characteristic electric field of TLS saturation, $\Phi$ is the complex digamma function, and $F$ is the filling factor of the TLS material. TLS are present in parts of the resonator (such as interfaces and dielectrics) and not others (such as superconductors and air), which effectively reduces the loss due to these systems. $F$ is the fraction of the resonator's total electrical energy stored in the TLS material. 

When more than one TLS medium is present, as is the case in the vast majority of physical circuits, $F \tan{\delta_{TLS}^0}$ in Eqn.~\ref{eqn:TLSloss} and \ref{eqn:TLSfreqshift} are replaced by a sum of contributions from each TLS material $\sum_{n} F_{n} \tan{\delta_{TLS,n}^0}$ where
\begin{equation}
    F_{n} = \frac{U_n}{U_{tot}} = \frac{\int_{V_n} \frac{\epsilon_n \lvert E^2 \rvert}{2}dV}{\int_V \frac{\epsilon \lvert E^2 \rvert}{2}dV}
\end{equation}
and $U_n$ is BLA...define all terms.

It is clear from Eqn.~\ref{eqn:TLSloss} and \ref{eqn:TLSfreqshift} that TLS-induced loss and frequency shift is dependent on geometry, through the filling factor $F$, as well as power, temperature, and frequency. Theoretical curves are plotted in Fig.~\ref{fig:TLSTheoCurves}. These curves demonstrate that TLS-induced loss is highest at low power and temperature and decreases as power and temperature increase and TLS become saturated. Since quantum information processing applications operate at single photons and millikelvin temperatures, TLS loss is maximized.

As shown in the equations above, $\tan{\delta_{TLS}^0}$ can be determined either by fitting measured loss $1/Q_i$ as a function of power at low temperature to Eqn.~\ref{eqn:TLSloss}, or by fitting the measured frequency shift $\delta f/f_0$ as a function of power to Eqn.~\ref{eqn:TLSfreqshift}. This is discussed in detail in Sec.~\ref{sec:experiments}.

\subsection{Quasiparticle Loss Due to Stray Infrared Light}
As mentioned above, thermally excited quasiparticles contribute negligibly to resonator loss in the quantum computing low temperature regime. Quantum experiments, however, find a non-equilibrium quasiparticle population that leads to loss and degradation of the quantum circuit. The source of these "excess" quasiparticles has been identified as pair-breaking from stray IR light. \cite{Barends2011} unambiguously show that resonator internal quality factors and qubit energy relaxation times can be significantly degraded by excess quasiparticles from stray IR radiation, as well as demonstrate how this influence can be fully removed by isolating the devices from the radiative environment using multistage shielding. \cite{kreikebaum2016optimization} also show a systematic study of the shielding effect and report similar results.

\subsection{Quasiparticle Loss Due to Microwave-induced Pair-breaking}
It is also found that microwave tones for resonator readout, although well below the gap frequency of the superconducting ($h\nu \ll 2\Delta$), can indirectly break pairs and generate excess quasiparticles at high power. In this process, a strong microwave tone can pump a quasiparticle from an energy level of $E \gtrsim \Delta$ to a ladder of higher energy levels $E + n \omega$ (n=1,2,3...). When such a quasiparticle reaches a high enough energy level and relaxes back to an energy level slightly above the gap, a pair-breaking phonon can be emitted which produces more quasiparticles. This quasiparicle multiplication process has been theoretically studied \citep{Goldie2012} and experimentally confirmed \citep{DeVisser2014}. Serniak et al 2018 in PRL, and Wang et al 2014 in nature comm.

\subsection{Radiative Loss}
Strictly speaking, radiative loss refers to the ``antenna'' effect that a resonator loses its energy through radiating into the free space. Embedding the device in a high-Q cavity can effectively eliminate the radiation loss to free space, as is done in 3D qubit architecture which has achieved record-long energy relaxation times \citep{Paik_PhysRevLett.107.240501}. Because most superconducting devices are mounted in a device box, radiative loss can be generalized to include the loss associated with induced current on normal metal far from the device. For example, a resonator can couple capacitively or inductively to the device box made from a normal metal (usually Cu or Au) and induce current there. This loss can be reduced by coating the backside of the chip with superconducting films \citep{Sandberg2013}, making the devices box from superconductors, or adopting a gradiometric circuit design. Add \citep{Sage2011}

\subsection{Vortex Loss}
 Vortices of trapped magnetic flux form islands of normal metal in an otherwise continuous superconducting film, and thus can dissipate power when current is present at the core of the vortex. A systematic study of microwave response of vortices was carried out by \cite{Song2009} on thin Re and Al films where they found the trapped flux can lead to substantial reductions in the internal quality factor. It is also known that wider superconducting traces are more susceptible to vortex trapping. By implementing vortex-pinning hole arrays \citep{Chiaro2016} and applying well-designed magnetic shielding, vortex loss can be greatly mitigated. To avoid increasing TLS participation, the separation between the vortex-pinning hole arrays and the CPW center pins should be at lease 6~$\mu$m \citep{bothner2011improving,Chiaro2016}. Some other works report that trenching a slot on the center strip of CPW resonator is another straight forward method for reducing loss due to trapped vortices \citep{song2009reducing} and  single vortices trapped at current anti-nodes of CPW resonators can reduce quasiparticle loss (\citep{nsanzineza2014trapping}). Although these vortex trapping techniques can help achieve higher $Q_i$ values, implementing them adds an extra level of complexity, whereas proper magnetic shielding is already promising for lowering the loss \citep{kreikebaum2016optimization} and is more easily adopted. 
%In general, one wants to minimize the magnetic field near the chip in order to minimize the loss due to on-chip magnetic vortices. However, on-chip vortex pinning can also be used. \cite{Song2009} shows that vortices can be pinned at designed on-chip sites away from devices, thus reducing the high power loss. People often use on chip holes fabricated on \cite{song2009reducing} shows that trenching a slot on the center strip of CPW resonator is another straight forward method for reducing loss due to trapped vortex.  \cite{nsanzineza2014trapping} reportsong2009reducings that single vortices trapped at current anti-nodes of CPW resonators can reduce quasiparticle loss.the metal ground plane to achieve that goal, but the separation between the holes and the CPW center pins should be at lease 6~$\mu$m to avoid increasing TLS participation \citep{Chiaro2016}. \cite{song2009reducing} shows that trenching a slot on the center strip of CPW resonator is another straight forward method for reducing loss due to trapped vortex.  \cite{nsanzineza2014trapping} reportsong2009reducings that single vortices trapped at current anti-nodes of CPW resonators can reduce quasiparticle loss. Although these vortex trapping techniques can help achieve higher $Q_i$ values, implementing them adds an extra level of complexity, whereas proper magnetic shielding is already promising for lowering the loss \citep{kreikebaum2016optimization} and is more easily adopted.


==> bulksubstratetable.tex <==
\begin{table*}
\caption{\label{tab:bulksubstratestable}Table of loss measurements of superconducting metals. Columns (from left to right): symbol denoting the measurement in Table~\ref{fig:review_scatter} (unlabelled), superconductor in measured device (SC), reference where measurement is reported (Reference), method of metal deposition (Dep.), surface treatments applied and etch type used to define resonators (Surf./Etch), substrate on which metal was deposited (Substrate), design of measured device (Geom.), reported low power loss $\tan{\delta_{LP}}$, reported intrinsic TLS loss $F \tan{\delta_{TLS}^0}$, and width $w$ of conductor and gap $g$ between conductor and ground plane. Therm. evap.: Thermal evaporation. MBE: Molecular beam epitaxy. PVD: Plasma vapor deposition. RIE: Reactive ion etch. H-pass.: hydrogen-passivated. $\mathrm{\lambda/2}$ or $\mathrm{\lambda/4}$: CPW resonator of length stated. LE IDC: Lumped element resonator with interdigitated capacitor. NA: information not available. Note: Values cannot be directly compared due to significant experimental differences.}
\begin{ruledtabular}
\begin{tabular}{cccccc}
Substrate & Reference & Growth & Geom. & $\tan{\delta_{LP}}$ & $F \tan{\delta^0_{TLS}}$ \\
& & & &[$\times 10^{-6}$]& [$\times 10^{-6}$] \\
\hline
%GaAs
%Si
$\mathrm{Al_2O_3}$ & \cite{Luiten1993} & Crystal & Cylinder &  & 1$\times 10^{-9}$\\
$\mathrm{Al_2O_3}$ & \cite{Krupka1999} & Crystal & Whispering-gallery rod &  & 1$\times 10^{-9}$\\
$\mathrm{YSZ}$ & \cite{Martinis2014} & Crystalline & CPW & 4 to 5$\times 10^{-4}$ & \\
$\mathrm{LSAT}$ & \cite{Martinis2014} & Crystalline & CPW & 7 to 9$\times 10^{-5}$ & \\
$\mathrm{MAO}$ & \cite{Martinis2014} & Crystalline & CPW & 1.2 to 1.8$\times 10^{-5}$ & \\
$\mathrm{SLAO}$ & \cite{Martinis2014} & Crystalline & CPW & 1.0 to 1.2$\times 10^{-5}$ & \\
$\mathrm{YAG}$ & \cite{Martinis2014} & Crystalline & CPW & < 1$\times 10^{-5}$ & \\
$\mathrm{YAO}$ & \cite{Martinis2014} & Crystalline & CPW & < 1$\times 10^{-5}$ & \\
$\mathrm{LAO}$ & \cite{Martinis2014} & Crystalline & CPW & < 1$\times 10^{-5}$ & \\
\end{tabular}
\end{ruledtabular}
\end{table*}

==> oldlosssection.tex <==
%Loss in a superconducting microwave resonator at low temperatures can be written as:
%\begin{equation}
%    \frac{1}{Q_{i}} = \tan{\delta} = F \tan{\delta_{TLS}} + \frac{1}{Q_{HP}}
%\end{equation}
%where $Q_{i}$ is the internal quality factor of the resonator and is equal to the inverse of the total loss in the resonator $\tan{\delta}$, $F \tan{\delta_{TLS}}$ is TLS loss, and $1 \over Q_{HP}$ is the sum of high power losses. High power loss is generally small and power-independent in the operational regime of a superconducting quantum circuit, whereas TLS loss has a distinct power dependence as well as a temperature dependence. 

%models of temperature and power dependence, their physical underpinnings, and the reasons why models are useful.

%\subsection{TLS Loss}
%Much is still uncertain about the origins and behavior of TLS \citep{Muller2017}. The general model for TLS loss in a weak electric field is \citep{Phillips}:
%\begin{equation}
%\label{eqn:TLSloss}
%    F \tan{\delta_{TLS}} = F \tan{\delta_{TLS}^0} {\tanh({\hbar \omega_0 \over 2 k_B T}) \over (1 + ({<n> \over n_c}))^\beta}.
%\end{equation}
%where $F$ is the filling factor of the TLS material, $\tan{\delta_{TLS}^0}$ is the TLS loss of the system at zero power and temperature ($<n> = 0$ and $T = 0$), $\omega_0$ is the resonance angular frequency, and $\beta$ is a variable determined by TLS population densities, but is usually close to 0.5. TLS become saturated at high powers, and therefore do not contribute to high power loss. As power decreases in the circuit, total TLS loss increases until it flattens off around single photon powers, near the critical photon number $<n_{c}>$. $\tan{\delta_{TLS}^0}$ can be seen as a materials constant, where each TLS material has an intrinsic $\tan{\delta_{TLS}^0}$ value associated with it. 

%The dielectric constant, and thus the resonance frequency, of the resonator is affected by TLS as \citep{Gao2008b}:
%\begin{equation}
%\label{eqn:TLSfreqshift}
%   \frac{\Delta f}{f_0} = -\frac{F}{2}\frac{\Delta \epsilon}{\epsilon} = -\frac{F \tan{\delta_{TLS}^0}}{\pi}[\Re{\Phi(\frac{1}{2}+\frac{1}{2 \pi i}\frac{\hbar \omega}{k T}) - \log{\frac{\hbar \omega}{k T}}}]
%\end{equation}
%where $\Delta f$ is the resonance frequency shift, $\Delta \epsilon$ is the dielectric constant shift, $\omega$ is the frequency, $\Phi$ is the complex digamma function.



%When more than one TLS material is present in a device, as is the case in the vast majority of physical circuits, $F \tan{\delta_{TLS}^0}$ can be broken down into the loss from each TLS material, as \citep{Calusine2018}:
%\begin{equation}
%    F \tan{\delta_{TLS}^0} = \sum_{n} p_{n} \tan{\delta_{TLS,n}^0}
%\end{equation}
%where $\tan{\delta_{TLS,n}^0}$ is the loss tangent of material or interface $n$, and $p_n$ is the participation ratio of this material or interface, given by:
%\begin{equation}
%    p_{n} = \frac{U_n}{U_{tot}} = \frac{\int_n \frac{\epsilon_n \lvert E^2 \rvert}{2}}{\int_V \frac{\epsilon_n \lvert E^2 \rvert}{2}}
%\end{equation}
%where $U_n$ is the electric field stored in material or interface $n$, $U_{tot}$ is the total electric field, $E$ is the local electric field, and $\epsilon_n$ is the dielectric constant of material or interface $n$.

%\subsection{High Power Loss}

%High power loss originates from a variety of sources including radiation, quasiparticles, magnetic fields, and conduction in normal metals. If measurements are taken with an improper experimental set-up, there is a risk of high power losses contributing significantly to low power loss or even dominating TLS loss at single photon power. For example, improper magnetic shielding can cause vortex loss to become significant \citep{Song2009}. Thus, high power loss measurements can be a crucial tool for obtaining accurate TLS loss values for materials of interest.

%A dearth of magnetic shielding can lead to the presence of an ambient magnetic field near the sample, trapping vortices on the chip surface within resonators. These vortices act as a high power loss channel \citep{Song2009}. \cite{Song2009} demonstrate that the internal quality factor of a resonator can be significantly reduced by the trapping of a small number of vortices.

%Radiation loss has been shown to be a significant factor in CPW resonators at high power. \cite{Sage2011} demonstrate that as the width and gap of a CPW resonator increase, the internal quality factor at high power decreases, indicating an increase in radiation loss to the environment. 

%\cite{Zmuidzinas2012} describes high power radiation loss $Q_{rad}$ as:
%\begin{equation}
%    Q_{rad} \sim 5 \times 10^{-3} (\lambda_0/W)^2
%\end{equation}
%where W is the resonator conductor width.

%Quasiparticles are unpaired electrons that act as a loss channel in superconductors. As on-chip temperature decreases, the density of quasiparticles decreases exponentially, until it reaches a low-temperature equilibrium \citep{Wilson2004}. \cite{Barends2008} show that the quasiparticle relaxation time becomes saturated at low temperature in resonators, which could be the result of a second relaxation channel other than the electron-phonon interaction.

%The presence of silver paint or other magnetic or normal materials can also contribute to high power loss.

%\subsection{Other Loss Mechanisms}

%Spurious modes such as box, chip, and slotline modes can muddy resonator measurements and decrease their accuracy. If these modes are at frequencies close to the resonance frequency of the resonator of interest, coupling can occur and they can act as a loss channel.

%Box modes are resonances sustained within the free space in the sample box where the superconducting quantum circuit chip is held during cryogenic measurement, the frequencies of which are dependent on box geometry as:
%\begin{equation}
%    f_{nml} = \frac{c}{2} \sqrt{ \frac{l^2 + n^2}{L^2} + \frac{m^2}{H^2} }
%\end{equation}
%where c is the velocity of light in vacuum, and $n,m,l$ denote the number of half wavelengths spanned by the electromagnetic field in the x-, y- and z-axis. By modifying the geometry or boundary
%conditions of the cavity, box modes can be increased or decreased in frequency. For example, adding an evacuated space below the chip raises the box modes \citep{Bejanin2016}. The addition of coaxial pogo pins has a similar effect %\citep{Bejanin2016,Bronn2018,Mcconkey2017}.

% Add chip modes, slotline modes

%Wirebond crosstalk can also pose an issue. \cite{Wenner2011} discusses the elimination of crosstalk from wirebonds by moving to a high density of short wirebonds.
